Supervised Learning in the Presence of Noise: Application in ICD-10 Code Classification

ICD coding is the international standard for capturing and reporting health conditions and diagnosis for revenue cycle management in healthcare. Manually assigning ICD codes is prone to human error due to the large code vocabulary and the similarities between codes. Since machine learning based approaches require ground truth training data, the inconsistency among human coders is manifested as noise in labeling, which makes the training and evaluation of ICD classifiers difficult in presence of such noise. This paper investigates the characteristics of such noise in manually-assigned ICD-10 codes and furthermore, proposes a method to train robust ICD-10 classifiers in the presence of labeling noise. Our research concluded that the nature of such noise is systematic. Most of the existing methods for handling label noise assume that the noise is completely random and independent of features or labels, which is not the case for ICD data. Therefore, we develop a new method for training robust classifiers in the presence of systematic noise. We first identify ICD-10 codes that human coders tend to misuse or confuse, based on the codes' locations in the ICD-10 hierarchy, the types of the codes, and baseline classifier's prediction behaviors; we then develop a novel training strategy that accounts for such noise. We compared our method with the baseline that does not handle label noise and the baseline methods that assume random noise, and demonstrated that our proposed method outperforms all baselines when evaluated on expert validated labels.

==> conf_paper/oracle_removed.tex <==
\subsection{Comparison with oracle methods}
\cheng{I recommend that we remove the entire subsection. It's so complex-- even I get completely lost}
It is questionable if the only problem of original labels is that they additionally include a symptom code when only the specific diagnosis code should be used. 
Then, if we have good classifiers that can predict the specific diagnoses, we may just remove the symptom codes from the predictions when any of the related specific diagnosis codes are predicted to exist. An immediate counter-argument would be that there are also instances where the original coders annotated only the symptom codes without using any specific diagnosis code, when validating coders annotated only specific diagnosis code for it. Taking a step further, we questioned if our proposed method does more than that. 

We experimented with a hypothetical `oracle' classifier which generates a ranked list based on the original labels. This could be considered as a simulation of evaluating the original coders based on validating coders criteria. 
If an instance is annotated with the target code according to the original labels, it is assigned a score 1. If not, it is assigned a score 0. 
The instances with the same score are randomly shuffled. We repeated the evaluation 1,000 times and reported the average. 

We also tested `fixed oracle' which scores an instance 1 only if the target symptom code is annotated without the related diagnosis code. If both the target symptom codes and related diagnosis code are annotated, it scores the instances 0.5. If none of them are annotated, it gets 0. 

\input{conf_paper/table/oracle}
The evaluation of these simulated models on validated labels are listed in table~\ref{tab:oracel}, along with the baseline and the proposed model. `fixed oracle's MAP was far from perfect, and even worse than the proposed classifier. Also, the gap between the proposed method and the baseline method was larger than the gap between `fixed oracle' and `oracle'. We believe this is because there are cases that the validated labels indicate the instance should only have a specific code, but the original label annotated the symptom code without any specific codes. 




==> conf_paper/table/oracle.tex <==

\begin{table}[]
\centering
\begin{tabular}{c|c|c}
\toprule
\textbf{Oracle}   & \textbf{Fixed Oracle} & \textbf{$\Delta$} \\ \hline
61.0             & 65.2                 & 4.2          \\ \hline \hline 
\textbf{Baseline} & \textbf{Proposed}     & \textbf{$\Delta$} \\ \hline
48.1             & 63.3                 & 15.2          \\ \bottomrule
\end{tabular}
\caption{Mean average precision of hypothetical oracle predictors and the models on validated labels. The original labels are used as oracle's predictions. Fixed oracle's predictions are also based on the original labels, but fixed by rules. The score differences of preceding two columns are listed under column $\Delta$. }
\label{tab:oracel}
\end{table}


==> conf_paper/table/oracle_full.tex <==
\begin{table*}[]
\centering
\begin{tabular}{c|c|c|c||c|c|c}
\toprule
 \textbf{Code}   & \textbf{Oracle}   & \textbf{Transform Oracle} & \textbf{$\Delta$}   & \textbf{Baseline} & \textbf{Proposed} &  \textbf{$\Delta$}     \\ \hline
M54.5                   & 0.263 & 0.609 & 0.346  & 0.350 & 0.795 & 0.446  \\
R10.9                   & 0.704 & 0.767 & 0.064  & 0.533 & 0.501 & -0.032 \\
R92.8                   & 0.516 & 0.537 & 0.021  & 0.661 & 0.687 & 0.026  \\
M54.2                   & 0.685 & 0.611 & -0.074 & 0.639 & 0.682 & 0.042  \\
R53.1                   & 0.816 & 0.817 & 0.001  & 0.698 & 0.733 & 0.035  \\
M25.561                 & 0.404 & 0.625 & 0.220  & 0.319 & 0.627 & 0.309  \\
M25.562                 & 0.654 & 0.657 & 0.003  & 0.272 & 0.621 & 0.349  \\
R10.2                   & 0.840 & 0.890 & 0.050  & 0.586 & 0.758 & 0.172  \\
M25.511                 & 0.448 & 0.494 & 0.046  & 0.758 & 0.958 & 0.200  \\
M79.671                 & 0.440 & 0.439 & -0.001 & 0.430 & 0.171 & -0.259 \\
M54.6                   & 0.688 & 0.678 & -0.009 & 0.183 & 1.000 & 0.817  \\
R11.2                   & 1.000 & 1.000 & 0.000  & 0.478 & 0.765 & 0.287  \\
R55                     & 0.345 & 0.350 & 0.005  & 0.729 & 0.063 & -0.666 \\
R41.0                   & 0.622 & 0.617 & -0.004 & 0.700 & 0.545 & -0.155 \\
R10.13                  & 1.000 & 1.000 & 0.000  & 0.000 & 0.500 & 0.500  \\
R09.89                  & 0.340 & 0.340 & 0.000  & 0.367 & 0.722 & 0.356  \\ \hline
\multicolumn{1}{c|}{MAP} & 0.610 & 0.652 & 0.042  & 0.481 & 0.633 & 0.152 

   \\ \bottomrule
\end{tabular}
\caption{Average precision of the models and original label-based oracle predictors on the validated labels. The score differences of preceding two columns are listed under column $\Delta$. }
\label{tab:oracel_full}
\end{table*}

==> conf_paper/table/sce_full.tex <==
\begin{table}[htbp]
\begin{tabular}{l|c|c}
\toprule
        & \textbf{Vanilla} & \textbf{Symmetric cross-entropy} \\ \hline 
R06.02  & 0.821   & 0.791                   \\
R05     & 0.902   & 0.916                   \\
M54.5   & 0.291   & 0.298                   \\
R10.9   & 0.554   & 0.512                   \\
R53.1   & 0.571   & 0.432                   \\
M25.561 & 0.371   & 0.360                   \\
M25.562 & 0.551   & 0.526                   \\
R10.2   & 0.665   & 0.598                   \\
M25.551 & 0.918   & 0.893                   \\
M25.552 & 0.752   & 0.776                   \\
M25.511 & 0.788   & 0.822                   \\
R10.11  & 0.802   & 0.757                   \\
R10.31  & 0.704   & 0.729                   \\
M25.512 & 0.548   & 0.579                   \\
M79.671 & 0.407   & 0.306                   \\
M54.6   & 0.616   & 0.639                   \\
M25.572 & 0.790   & 0.770                   \\
R10.32  & 0.620   & 0.698                   \\ \hline
MAP     & 0.65    & 0.63                   \\ \bottomrule
\end{tabular}
\caption{Experiment result when noisy robust method symmetric cross-entropy is applied~\cite{sce}. Symmetric cross-entropy does not out-perform the vanilla method. This experiment was done with a different split than Table 6, so not directly comparable. }
\end{table}
